ConfigBot: Adaptive Resource Allocation for Robot Applications in Dynamic Environments

The growing use of service robots in dynamic environments requires flexible management of on-board compute resources to optimize the performance of diverse tasks such as navigation, localization, and perception. Current robot deployments often rely on static OS configurations and system over-provisioning. However, they are suboptimal because they do not account for variations in resource usage. This results in poor system-wide behavior such as robot instability or inefficient resource use. This paper presents ConifgBot, a novel system designed to adaptively reconfigure robot applications to meet a predefined performance specification by leveraging \emph{runtime profiling} and \emph{automated configuration tuning}. Through experiments on multiple real robots, each running a different stack with diverse performance requirements, which could be \emph{context}-dependent, we illustrate ConifgBot's efficacy in maintaining system stability and optimizing resource allocation. Our findings highlight the promise of automatic system configuration tuning for robot deployments, including adaptation to dynamic changes.

==> _macros.tex <==
\RequirePackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot}
\def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} 
\def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} 
\def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} 
\def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} 
\def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

\newcommand{\circled}[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {#1};}}
\newcommand{\tick}{\ding{51}}
\newcommand{\cros}{\ding{55}}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}


\newcommand{\cgroup}{\texttt{cgroup}\xspace}
\newcommand{\cgroups}{\texttt{cgroups}\xspace}

\definecolor{darkgreen}{RGB}{0,100,0}
\newcommand{\greencheck}{\textcolor{darkgreen}{\checkmark}}
\newcommand{\redcross}{\textcolor{red}{$\times$}}

\newcommand{\system}{\textsc{ConfigBot}\protect\kern-.1em\xspace}
\newcommand{\robotStack}[1]{\textsc{\textbf{#1}}}


\newcommand{\badResult}[1]{\textcolor{red}{#1 \textbf{\texttimes}}}
\newcommand{\goodResult}[1]{\textcolor{green}{#1 \textbf{\checkmark}}}


\DeclareRobustCommand{\adaptor}{\raisebox{-0.2\height}{\includegraphics[height=1em]{figures/adaptor_arrow.png}}}

\newcommand{\aditya}[1]{}
\newcommand{\chris}[1]{}
\newcommand{\dk}[1]{}
\newcommand{\joydeep}[1]{}
\newcommand{\rohit}[1]{}
\newcommand{\sadanand}[1]{}


\renewcommand{\aditya}[1]{{\color{red}\textbf{[aditya]:} #1}}
\renewcommand{\chris}[1]{{\color{violet}\textbf{[chris]:} #1}}
\renewcommand{\dk}[1]{{\color{brown}\textbf{[daehyeok]:} #1}}
\renewcommand{\joydeep}[1]{{\color{purple}\textbf{[joydeep]:} #1}}
\renewcommand{\rohit}[1]{{\color{blue}\textbf{[rohit]:} #1}}
\renewcommand{\sadanand}[1]{{\color{olive}\textbf{[sadanand]:} #1}}

\newcommand{\pnc}{\textsf{PNC}\protect\kern-.1em\xspace}
\newcommand{\csr}{\textsf{CSR}\protect\kern-.1em\xspace}




